Automatic Sequences and Zip-Specifications

We consider infinite sequences of symbols, also known as streams, and the decidability question for equality of streams defined in a restricted format. This restricted format consists of prefixing a symbol at the head of a stream, of the stream function `zip', and recursion variables. Here `zip' interleaves the elements of two streams in alternating order, starting with the first stream. For example, the Thue-Morse sequence is obtained by the `zip-specification' {M = 0 : X, X = 1 : zip(X,Y), Y = 0 : zip(Y,X)}. Our analysis of such systems employs both term rewriting and coalgebraic techniques. We establish decidability for these zip-specifications, employing bisimilarity of observation graphs based on a suitably chosen cobasis. The importance of zip-specifications resides in their intimate connection with automatic sequences. We establish a new and simple characterization of automatic sequences. Thus we obtain for the binary zip that a stream is 2-automatic iff its observation graph using the cobasis (hd,even,odd) is finite. The generalization to zip-k specifications and their relation to k-automaticity is straightforward. In fact, zip-specifications can be perceived as a term rewriting syntax for automatic sequences. Our study of zip-specifications is placed in an even wider perspective by employing the observation graphs in a dynamic logic setting, leading to an alternative characterization of automatic sequences. We further obtain a natural extension of the class of automatic sequences, obtained by `zip-mix' specifications that use zips of different arities in one specification. We also show that equivalence is undecidable for a simple extension of the zip-mix format with projections like even and odd. However, it remains open whether zip-mix specifications have a decidable equivalence problem.

==> mix-zip.tex <==

\begin{definition}
  Let $\aspec$, $\bspec$ be stream specifications.
  We call $\aspec$ and $\bspec$ \emph{equivalent}, denoted $\aspec \sim \bspec$, if \todo{they produce the same stream}.
  \todo{Move to section on zip specifications; there we also need a definition of pure}.
\end{definition}

We introduce a special unproductive stream constant $\Omega$
with the equation $\Omega \to \Omega$.
This allows us to represent stream terms with finite production:
$a_1 : \ldots : a_n : \Omega$ with data elements $a_1,\ldots,a_n$ and $n\in\nat$.
We call these terms \emph{list representations}.


\begin{definition}\normalfont
  Let $\acxt$ and $\bcxt$ be multi-hole stream contexts with holes $\cxthole_1,\ldots,\cxthole_k$.
  Then $\bcxt$ is called \emph{substitutable for $\acxt$}
  if for all list representations $\ell_1,\ldots,\ell_k$ it holds: whenever
  \begin{align*}
    C[\ell_1,\ldots,\ell_k] &\mred a_1 : \ldots : a_n : s
  \end{align*}
  for some $a_1,\ldots,a_n,s$, then
  \begin{align*}
    D[\ell_1,\ldots,\ell_k] &\mred a_1 : \ldots : a_n : s'
  \end{align*}
  for some $s'$.
  Furthermore, $C$ and $D$ are called \emph{equivalent} if $C$ and $D$ are substitutable for each other. 
\end{definition}

\begin{lemma}
  For every $n \in \nat$, the context $\cxthole_1$ is equivalent to 
  \begin{align*}
    \zipn{n}{\pjx{0}{n}{\cxthole_1},\ldots,\pjx{n-1}{n}{\cxthole_1}}
  \end{align*}
\end{lemma}

\begin{definition}\normalfont
  Let $\aspec$ a zip-specifications with root $\rootsc$,
  and $C$ be a stream context.
  Let $C[\aspec]$ be obtained from $\aspec$
  by adding a fresh root $\rootsc'$ with defining equation $\rootsc' = C[\rootsc]$.
  %
  For a~set of contexts $\mcl{C}$ and a set of specifications $\specclass$,
  we define:
  \begin{align*}
  \mcl{C}[\specclass] = \{\, C[t] \mid C \in \mcl{C},\; \aspec \in \specclass \,\}
  \end{align*}
  Then $\specclass$ is called \emph{closed under $\mcl{C}$} if 
  for every $C \in \mcl{C}$ and~$\aspec \in \specclass$, 
  there exists $\aspec' \in \specclass$ such that $\aspec'$ is equivalent to $C[\aspec]$.
\end{definition}

We define two sets of contexts:
\begin{align*}
  \cxtmod &= \{\, \pjx{i}{n}{\cxthole} \where i,n \in \nat \,\}\\
  \cxtzip &= \{\, \zipn{n}{\zeros,\ldots,\zeros,\underbrace{\cxthole}_{\text{$i$-th}},\zeros,\ldots,\zeros} \where i \le n \in \nat \,\}
\end{align*}
For every $k \in \nat$ we let $\zipk{k}$ be the set of zip-$k$ specifications.

\begin{proposition}\label{prop:mod:zip}
  For all $i,n,k\in\nat$ with $n,k \ge 1$, and all streams $\astr_0,\ldots,\astr_{k-1}$: 
  \begin{align*}
    &\pjx{i}{n}{
      \zipn{k}{\astr_0,\ldots,\astr_{k-1}}
    } =
      \\
    &\zipn{k}{ 
        \pjx{\floor{f(0)/k}}{n}{\astr_{\modulo{k}{f(0)}}},
        \ldots,
        \pjx{\floor{f(k-1)/k}}{n}{\astr_{\modulo{k}{f(k-1)}}}
                 }
  \end{align*}
  where $f(z) = i + z n$.
\end{proposition}

\begin{lemma}
  The set $\zipk{k}$ is closed under $\cxtmod$.
\end{lemma}
%
\begin{proof}
  \todo{D: Here we could use that $k$-automaticity is closed under arithmetic subsequences, 
    or is the commented out (unfinished) proof an improvement over existing ones?}
%   Let $\aspec \in \zipk{k}$ over variables $\conset = \{M_0,\ldots,M_n\}$
%   and $C = \pjx{m}{p}{\cxthole} \in \cxtmod$ with $m,p \in \nat$.
%   Theorem~\ref{thm:dform} allows us to assume that $\aspec$ is in D normal form:
%   \begin{align*}
%     \acon_i = a_i : \zipn{k}{\acon_{i,0},\ldots,\acon_{i,k-1}} \quad \text{for every $0 \le i \le n$}
%   \end{align*}
%   Define the specification $\bspec$ to consist of:
%   For every $\acon_i \in \conset$ and $j \le m + 2p \in \nat$ let
%   $\acon_i^{(j)}$ be fresh, and define
%   {\belowdisplayskip2pt
%   \begin{align*}
%     \acon_i^{(j)} = \underbrace{a_i :}_{\text{drop if $j>0$}} \zipn{k}{\acon_{i,\modulo{k}{f_j(0)}}^{(\floor{f_j(0)/k})},\ldots,\acon_{i,\modulo{k}{f_j(k-1)}}^{(\floor{f_j(k-1)/k})}}\\
%     \text{where } f_j(z) = z p + \begin{cases}j-1&\text{if $j>1$}\\p-1&\text{if $j=0$}\end{cases}
%   \end{align*}}%
%   \\[.5ex]
%   where $\acon_i^{(m)}$ is the root of $\bspec$.
%   %
%   We have that $\floor{f_j(0)/k} \le \ldots \le \floor{f_j(k-1)/k} \le \lfloor \max (j-1,p-1)/k +p \rfloor \le m+2p$.
%   Thus all variables in the right-hand sides are defined.
%   
%   Employing Proposition~\ref{prop:mod:zip}
%   it is now straightforward to show that $\pjx{j}{p}{\acon_i} \sim \acon_i^{(j)}$.
%   Hence, we get $\pjx{m}{p}{\aspec} \sim \bspec$.
\end{proof}

% not used
% \begin{lemma}
%   The set $\cxtzip[\zipk{k}]$ is closed under $\cxtmod$ and $\cxtzip$.
% \end{lemma}
% 
% \begin{proof}
% \end{proof}

The following theorem states that automatic sequences can
be compared with zip-mix-specifications:
\begin{theorem}
  Let $k \in \nat$, $\aspec \in \zipk{k}$ and $\bspec \in \zipmix$.
  Then the equivalence of $\aspec$ and $\bspec$ is decidable.
\end{theorem}
%
\begin{proof}
  \newcommand{\eqset}{\Psi}
  Let $\bspec$ be over variables $\mcl{N} = \{\bcon_0,\ldots,\bcon_{n-1}\}$.
  Then Theorem~\ref{} allow us to assume that 
  all equations of $\bspec$ are of one of the forms:
  \begin{align}
    \bcon_j &= a_j: \bcon_{j,0} \label{form:cons}\\
    \bcon_j &= \zipn{\ell_j}{\bcon_{j,0},\ldots,\bcon_{j,\ell_j-1}} && \text{for some $\ell_j\in\nat$} \label{form:zip}
  \end{align}
  for $0 \le j \lt n$. 
  Define the set $\eqset$ consist of all equations of the form $\bcon = \cspec$
  with $\bcon \in \mcl{N}$ and $\cspec$ a $\zipk{k}$-specification.
  We define a proof system 
  for statements of the form `$\Delta \vdash e$'
  where $\Delta \subseteq \eqset$ and $e \in \eqset$:
  for $0 \le j < n$ we define\vspace{.5ex}
  \begin{gather*}
    \infer[\text{$N_j = \cspec' \in \Delta$ and $\cspec \sim \cspec'$}]{
      \Delta \vdash \bcon_j = \cspec
    }{
    }\\[.75ex]
    \infer[\text{case~\eqref{form:cons}}]{
      \Delta \vdash \bcon_j = \cspec
    }{
      \head{\bcon_j} = \head{\cspec}
      &
      \Delta \vdash \bcon_{j,0} = \pjx{1}{1}{\cspec}
    }\\[.25ex]
    \infer[\text{case~\eqref{form:zip}}]{
      \Delta \vdash \bcon_j = \cspec
    }{
      \Delta \vdash \bcon_{j,0} = \pjx{0}{\ell_j}{\cspec}
      &\ldots&
      \Delta \vdash \bcon_{j,\ell_j-1} = \pjx{\ell_j-1}{\ell_j}{\cspec}
    }
  \end{gather*}
  Then $\aspec \sim \bspec$ if and only if $\setemp \vdash \bcon_{0} = \aspec$.
\end{proof}

